Monte-Carlo Tree Search as Regularized Policy Optimization

The combination of Monte-Carlo tree search (MCTS) with deep reinforcement learning has led to significant advances in artificial intelligence. However, AlphaZero, the current state-of-the-art MCTS algorithm, still relies on handcrafted heuristics that are only partially understood. In this paper, we show that AlphaZero's search heuristics, along with other common ones such as UCT, are an approximation to the solution of a specific regularized policy optimization problem. With this insight, we propose a variant of AlphaZero which uses the exact solution to this policy optimization problem, and show experimentally that it reliably outperforms the original algorithm in multiple domains.

==> recycle bin/old_intro.tex <==
%There is a natural dichotomy of solution methods for reinforcement learning (RL): model-based and model-free methods \citep{sutton_RLIntro_1998}. By construction, model-based methods are designed to extract dynamics information from the environment, and enables learning with high sample efficiency even on challenging image-based domains \citep{kaiser2019model}. On the other hand, model-free methods focus on domain-agnostic quantities such as Q-functions \citep{mnih2013playing,kapturowski2018recurrent} and policy \citep{schulman2015trust,mnih2016asynchronous,schulman2017proximal,song2019v}, without explicitly leveraging information about the dynamics. Despite a seemingly coarse treatment of rich information from the environment, with careful designs of algorithms and scaling up to high-performing computational architectures, model-free methods still achieve de-facto state-of-the-art results on benchmark domains \citep{kapturowski2018recurrent,song2019v}.

%Arguably, efficient hybrid RL algorithms should exploit the best from both worlds.

%Designing efficient RL algorithms requires investigating the link between model-free and model-based algorithms.

%Model-free and model-based methods have strengths in quite different aspects. For example, in cases where agents are required to reason over long horizons \citep{guez2018learning}, model-based planning achieves significantly higher asymptotic performance than model-free learning. 

%, of which AlphaZero is a highly successful example \citep{silver2017mastering}. AlphaZero alternates between highly efficient model-based tree search and model-free learning

%[Yunhao: introduce expert iteration; I have written some pieces but need to stitch them together better]

 %To make the best of both paradigms, a recent trend is to combine both model-free and model-based methods. For example, model-free algorithms could potentially speed up learning by bootstrapping imaginary samples generated from learned models \citep{gu2016continuous,weber2017imagination,nagabandi2018neural}. [do a transition into expert iteration] 
 
Deep reinforcement learning (RL) has been highly successful in solving an increasing large number of tasks~\citep{mnih2013playing, mnih2015human, silver2016mastering, levine2016end, OpenAI_dota, alphastar}.

Along with architectural improvements such as distributed agents~\citep{nair2015massively,espeholt2018impala,kapturowski2018recurrent}, state-of-the-art of model-free deep RL algorithms have been driven by better understanding of algorithmic issues such as trust region optimization~\citep{schulman2015trust,abdolmaleki2018maximum} and off-policyness~\citep{munos2016safe,espeholt2018impala}. In particular, mathematical insights into practical issues of policy gradient techniques~\citep{sutton2000policy} led to advanced policy optimization techniques such as
trust region policy search ~\citep{schulman2015trust,schulman2017proximal,abdolmaleki2018maximum,song2019v}, deterministic policy gradients ~\citep{silver2014deterministic,lillicrap2015continuous} and off-policy policy gradients ~\citep{wang2016sample,espeholt2018impala}. These successive improvements pushed up state-of-the-art performances on various benchmark domains.

%TRPO~\citep{schulman2015trust}, PPO~\citep{schulman2017proximal} or MPO~\citep{abdolmaleki2018maximum,song2019v} that all established a new state-of-the-art level of performance.

Concurrently, AlphaZero~\citep{silver2016mastering,silver2017mastering,schrittwieser2019mastering} established  new state-of-the-art results as a model-based RL algorithm, with significant performance gains over advanced model-free algorithms on benchmarks such as board games and Atari games~\citep{bellemare2013arcade}. Central to the success of AlphaZero is an highly efficient model-based planning subroutine \emph{Monte-Carlo Tree Search} (MCTS). To balance exploration and exploitation during planning, traditional designs of MCTS heuristics heavily draw inspirations from well established bandit literature~\citep{kocsis2006bandit}. Interestingly, however, practical implementations of MCTS could involve seemingly ad-hoc design choices, which are handcrafted to achieve success on specific tasks \citep{silver2017mastering,schrittwieser2019mastering}. Notably, AlphaZero incorporates the prior distribution predicted by a policy network into the search procedure (see \Cref{sec:background}), a critical design unseen in previous MCTS algorithms such as UCT~\citep{kocsis2006bandit}.

Despite the high performance of AlphaZero, its unique design on MCTS is not yet properly analyzed nor theoretically justified. This makes it hard to extend the algorithm and to build on its success. It is tempting to ask, what is an intuitive yet principled interpretation of the search heuristics employed by AlphaZero? 

\paragraph{Main idea} We show that AlphaZero performs a form of policy optimization that closely resembles state-of-the-art model-free policy optimization algorithms~\citep{abdolmaleki2018maximum,song2019v}. Specifically, we show that AlphaZero's unique design of MCTS search heuristics results in a policy that approximates the solution to a regularized policy optimization problem. With these insights, we propose a modified version of AlphaZero, which provides significant performance gains compared to the original algorithm, especially in certain cases where AlphaZero has been observed to fail \citep{hamrick2019combining}.

%We then leverage this connection to bring insights from the policy optimization literature into AlphaZero, and propose a modified version of the algorithm that offers improved performance when the number of expanded tree nodes in MCTS is limited.

Our paper proceeds as follows. In \Cref{sec:background}, we introduce background on general MCTS-based algorithms with a focus on AlphaZero. Then we provide a short summary of model-free policy optimization algorithms. In \Cref{sec:mcts_as_po}, we make the critical observation of the paper: AlphaZero (and more general MCTS-based algorithms) compute approximate solutions to a family of regularized policy optimization problems. With these insights, in  \Cref{sec:algo}, we propose a modified version of AlphaZero which leverages the benefits of policy optimization formalism in contexts where vanilla AlphaZero might fail. Finally, in \Cref{sec:experiments} we show that the modified algorithm outperforms AlphaZero on the Atari domain, as well as continuous control tasks.
%However, as a hybrid model-based \& model-free algorithm, AlphaZero does not possess all desired properties. To achieve high performance, AlphaZero relies on relatively high budgets of simulations for the tree search. Indeed, prior works  \citep{hamrick2019combining} have observed that AlphaZero suffers in cases where simulation budgets are low relative to the branching factor of the environment. To render the hybrid algorithm less sensitive to the simulation budgets is desirable: \textbf{(1)} Simulations can be computationally expensive, reducing the simulation budgets can greatly improve the training speed; \textbf{(2)} In environments where the branching factor is huge, it is not feasible to set up very high simulation budgets.

%We propose POZero, an extension of AlphaZero which performs well even under small simulation budgets. Our algorithmic improvement is based on a critical observation: AlphaZero's search procedure could be interpreted

% \todoin{have something good here. Probably critical part of the paper: we need to tease the reader and give her the will to read through the paper. Right now just putting something bad but at least we can start from something. \\ Yunhao: yes, probably come back after a larger part of the paper is done. Need just a couple of sentences to summarize the idea and entice the readers.}
%The critical observation is that successful MCTS algorithm as AlphaZero and UCT use an action selection formula that can be interpreted as trying to get the empirical visit count as close to a soft-max over the search Q-value that we note $\pibar$. The empirical visit count plays a critical role in the AlphaZero algorithm and we will argue why using the soft-max distribution $\pibar$ in place of the visit count makes more sense and prove it with experiments on the Atari test domain and control tasks. More importantly by using this soft-max $\pibar$ in place of the visit count we draw a link between exists model free algorithms and successful model based methods. We show that AlphaZero is close to standard policy optimization using estimation of Q-values coming from search while the search is also close to a policy optimization algorithm operating on imagined trajectories.  

%We will start in \cref{sec:background} by introducing some background on MCTS, particularly AlphaZero, and policy optimization aong with notations. From this we will introduce in \cref{sec:mcts_as_po} a soft-max over Q-values for different regularizers which relate to previous work on policy optimization and mirror descent and show how this relates to AlphaZero and UCT action selection formula. We then use this in \cref{sec:algo} to propose some slight modifications to AlphaZero which link it to policy optimization and argue about the of these change. Finally we provide experimental validations in \cref{sec:experiments} on the Atari domain and continuous control tasks.  

==> recycle bin/old_section_2.tex <==
\section{Background and notation}
\todoin{Yunhao: how about just Background?}
\label{sec:background}
Consider a Markov Decision Process (MDP) with state space $\mathcal{X}$ and action space $\mathcal{A}$. Let policy $\pi(\cdot|x)$ be a distribution over actions conditional on state $x$. At a discrete time $t \geq 0$, the agent in state $x_t$ takes action $a \sim \pi(\cdot|x_t)$, receives reward $r_t$, and transitions to a next state $x_{t+1} \sim p(\cdot|x_t,a_t)$. For simplicity, we always assume that there is a single initial state $x_0 \in \mathcal{X}$ and the RL objective is the discounted cumulative return $J(\pi) = \mathbb{E}_{\pi,x_0}[\sum_{t\geq 0}r_t\gamma^t]$ under policy $\pi$, with discount factor $\gamma\in (0,1)$. Let $Q^\pi(x,a)$ be the action value function (Q-function) from state $(x,a)$ under policy $\pi$. For control purpose, we aim to search for $\pi^\ast = \arg\max_\pi J(\pi)$.

To scale the optimization to high-dimensional state-action space, it is common practice to parameterize the policy $\pi_\theta(a|x)$ by a neural network $\theta$. Below we introduce several important algorithms for optimizing the parameterized policy $\pi_\theta(a|x)$.

\paragraph{Notations.} We introduce vector notations to simplify the presentation. For example, we use the bold font  $\mathbf{q} \in \mathbb{R}^{|\mathcal{A}|}$ to denote the vector Q-function $Q(x,a)$ such that $\mathbf{q}[a] = Q(x,a)$. Similarly, when contexts are clear $\pi_\theta$ could denote either the vector $\mathbf{\pi}_\theta\in \mathbb{R}^{|\mathcal{A}|}$ or the abstract policy $\pi_\theta$. For convenience, we always remove the notation's dependency on state $x$.

\subsection{AlphaZero \& MuZero}
\label{sec:alphazero_muzero}
There are a number of prior works which combine model-based planning with model-free deep learning \cite{anthony2017thinking,silver2017mastering, guez2018learning}. For simplicity, we focus on   
AlphaZero \citep{silver2017mastering}. AlphaZero could be interpreted as a special case of generalized policy improvement (GPI) \citep{sutton_RLIntro_1998}. In the general scheme of GPI, the algorithm alternates between policy improvement and policy evaluation. In AlphaZero, both steps are carried out during a local tree search, where the algorithm starts from a particular state $x$ and optimizes for a local policy $\pi_{\text{mcts}}(\cdot|x)$ via Monte-Carlo Tree Search (MCTS) \citep{browne2012survey}. Then the optimized local policy is distilled into the parameterized policy $\theta = \argmin_\theta \EEs{x}{D(\pi_\theta(\cdot|x), \pi_{\text{mcts}}(\cdot|x))}$ by minimizing certain divergence $D(\cdot,\cdot)$ with $\theta$. In turn, the distilled parametrized policy $\pi_\theta$ will inform the local search, further improving the local policy during next iterations. Below, we provide a quick overview on the two core components of AlphaZero: \textbf{Search} and \textbf{Learning}.

\paragraph{Search.} 
The search subroutine builds a tree where each nodes represents a state and has $|\mathcal{A}|$ children, one for each action. Traversing the tree from the root to a leaf is equivalent to generating a partial trajectory from the MDP, by executing a sequence of actions corresponding to traversed edges\footnote{Importantly, here the build-up of the search tree implicitly assumes that the transition $x_{t+1} \sim p(\cdot|x_t,a_t)$ is deterministic. Indeed, for applications such as board games and Atari games, the transitions are deterministic \citep{schrittwieser2019mastering}. There are methods to account for stochastic transitions, which we leave out of the presentation here. \todoin{add "causally correct" citation when its out on arxiv}}. New nodes $x$ comes with an estimated value $v_\theta(x)$ and policy $\pi_\theta(\cdot|x)$ computed by a neural network with weights $\theta$. The search proceeds by generating $n_{\text{sim}}$ simulations. In each simulation, the search traverses the tree from the root node until it reaches a leaf which is expanded by adding all of its children to the tree. Each node $x$ also maintains several statistics: the visit count $N(x,a)$ and the Q-function $Q(x,a)$ which are the amount of time a simualtion executed action $a$ from node $x$ and the average values of these simulation. 

During the forward traversal, for any node $x$ the action is selected according to

% The search subroutine builds a search tree $\mathcal{\mathcal{N},\mathcal{E}}$ with a MDP state $x_0$ as the root node $n(x_0) \in \mathcal{N}$. Each node $n(x) \in \mathcal{N}$ represents a real MDP state $x$ and each edge $e(a)\in \mathcal{E}$ represents a valid action $a\in \mathcal{A}$. By construction, each node $n(x)$ has $|\mathcal{A}|$ child nodes, representing $|\mathcal{A}|$ future transitions, and each child could be conveniently identified as the pair $(x,a)$. Traversing the tree from the root node to a leaf node is equivalent to generating a partial trajectory from the MDP state $x_0$, by executing a sequence of actions corresponding to traversed edges. Each node $n(x)$ maintains several statistics: the visit count $N(x,a)$, Q-function $Q(x,a)$ and a prior policy $P(x,a)$ of its child nodes. 

% The search proceeds by generating $n_{\text{sim}}$ simulations: in each simulation, the search traverses the tree, expands a child node and back-ups values of nodes along the traversed path. 


\begin{align}
    \argmax_a \brkt{Q(x,a) + c \cdot \pi_\theta(a|x) \cdot \frac{\sqrt{\sum_b N(x,b)}}{1 + N(x,a)}}
    %\cdot \nonumber \\(c_1 + \log (\frac{\sum_b N(x,b) + c_2 + 1}{c_2}))]. 
    \label{eq:azselection}
\end{align}
with $c$ being a numerical constant\footnote{In \cite{schrittwieser2019mastering} $c$ weakly depends on $\sum_b N(x,b)$ but for simplicity we will consider it constant like in \cite{silver2017mastering}}. 
Intuitively, the action selection rule aims to strike a balance between exploration and exploitation: the selection rule prefers actions with large potentials (large Q-value $Q(x,a)$ and prior $\pi_\theta(a|x)$) yet under-explored (small visitation counts $N(x,a)$). 

To rewrite the action selection formula, we introduce some notations below. First, we define an empirical visit count $\pihat$ where an additional visit count is added to each action
\begin{align}
    \pihat(a|x) \eqdef \frac{1 + N(x,a)}{|\mathcal{A}| + \sum_{b} N(x,b)}.
    \label{eq:pihat}
\end{align}
Further, let  
   $ \lambda \eqdef c\sqrt{\sum_b N(x,b)} / (|\mathcal{A}| + \sum_b N(x,b))$. We are now ready to rewrite the action selection formula (\ref{eq:azselection}) as
\begin{align}
    \argmax_a Q(x,a) + \lambda \cdot \frac{\pi_\theta(a|x)}{\pihat(a|x)}.
    \label{eq:az_act_select_reformalized}
\end{align}
For two vector $\mathbf{u}, \mathbf{v}$ we note $\prth{\frac{\mathbf{u}}{\mathbf{v}}}[a] = \frac{\mathbf{u}[a]}{\mathbf{v}[a]}$, so that the term inside the $\arg\max$ in \cref{eq:az_act_select_reformalized} can be written as 
\begin{align}
    \mathbf{q} + \lambda \frac{\mathbf{\pi}_\theta}{\mathbf{\pihat}}
    \label{eq:az_act_select_vector}
\end{align}
\todoin{Yunhao: what do we want to show with the vector notation here? Could we delay this equation to later?}

Another popular action selection formula is UCT \cite{kocsis2006bandit} as follows
\begin{align}
    \argmax_a \brkt{Q(x,a) + c \cdot \sqrt{\frac{\log\prth{\sum_b N(x,b)}}{1 + N(x,a)}}\;}.
    %\cdot \nonumber \\(c_1 + \log (\frac{\sum_b N(x,b) + c_2 + 1}{c_2}))]. 
    \label{eq:uctselection}
\end{align}
The main difference bwtween AlphaZero action selection formula (\ref{eq:azselection}) and UCT (\ref{eq:uctselection}) is the use of the prior $\pi_\theta(a|x)$. 

\todoin{the subsection (AZ search + UCT description probably should be shorter. The reader should already have an idea what is MCTS}
\todoin{can we remove some notation? For instance maybe remove $x$ as notation and note $\pi(a)$ instead of $\pi(a|x)$?}

% During the search, the algorithm could generate downstream nodes with a perfect simulator \citep{silver2017mastering} or with a learned model \citep{schrittwieser2019mastering}. With a learned model, the overall algorithm is called MuZero. We leave the details of MuZero in the Appendix. \todoin{add in appendix}

\paragraph{Learning.} As mentioned above, the search consists of $n_{\text{sim}}$ simulations, each generating a tree traversal starting from the root node $x_\text{root}$. This forms an empirical visitation distribution of the $|\mathcal{A}|$ actions at the root,
\begin{align}
    \frac{N(x_\text{root},a)}{\sum_{b} N(x_\text{root},b)}.
    \label{eq:azpihat}
\end{align}
 Since the search is meant to generate an optimized local policy, ideally we should expect this empirical visit count to improve upon e.g. the prior $\pi_\theta(a|x)$. However, this local policy is represented in a tabular way and does not allow for generalization to other unseen states. To distill the knowledge of the local policy into the parametric policy, AlphaZero reduces the following expected KL-divergence by gradient descent on $\theta$: 
\begin{align}
    \mathbb{E}_{x_\text{root}}\Big[\mathbb{KL}\brkt{\frac{N(x_\text{root},\cdot)}{\sum_{b} N(x_\text{root},b)}, \pi_\theta(\cdot|x_\text{root})}\Big],
    \label{eq:azlearning}
\end{align}
where $x_\text{root}$ is sampled from a distribution over states, e.g., from a prioritized replay buffer.

\subsection{Policy optimization}

Now, it is useful to take a step back and review the basic setup of policy optimization. Though the objective of policy optimization is to search for a globally optimal policy $\pi_\theta(a|x)$, practical algorithms always decompose the global optimization into a sequence of iterative updates. In each iteration, with current policy $\pi_\theta$, a generic local policy optimization problem at state $x$ is the following
\begin{align}
\max_{\mathbf{y} \in \mathcal{S}}  \ \mathcal{Q}^T \mathbf{y} - \mathcal{R}\prth{\mathbf{y}, \pi_\theta},
\label{eq:po_opt}
\end{align}
where $\mathcal{Q}[a] \approx Q^{\pi_\theta}(x,a)$ is an estimate of the Q-function under policy $\pi_\theta$,  $\mathcal{S}$ is the $|\mathcal{A}|$-dimensional simplex and $\mathcal{R}: \mathcal{S}^2 \mapsto \mathbb{R}$ a convex regularization term. The intuition of eq. (\ref{eq:po_opt}) is clear, we seek a local policy $\mathbf{y}$ which maximizes the value $Q^T\mathbf{y}$ while accounting for the regularization $\mathcal{R}(\mathbf{y},\pi_\theta)$.

Despite its simplicity, eq. (\ref{eq:po_opt}) summarizes a large spectrum of popular policy optimization algorithms. Indeed,
without the regularization $\mathcal{R}(\mathbf{y},\pi_\theta)=0$, eq. (\ref{eq:po_opt}) reduces to policy iteration \citep{sutton_RLIntro_1998}. In practice, it is beneficial to introduce non-trivial regularizations which stabilize/speed up the optimization. For example, trust region policy search \citep{schulman2015trust,schulman2017proximal,abdolmaleki2018maximum,song2019v} sets $\mathcal{R}(\mathbf{y},\pi_\theta)$ to be the KL-divergence; maximum entropy RL 
\cite{ziebart2010modeling, fox2015taming, o2016combining, haarnoja2017reinforcement} sets $\mathcal{R}(\mathbf{y},\pi_\theta)$ to be the entropy of $\mathbf{y}$ to encourage exploration. In addition, when $\mathbf{y}$ is updated from $\pi_\theta$ via gradient descent (instead of optimizing (eq. \ref{eq:po_opt}) fully), the above formulation reduces to (regularized-)policy gradient \citep{sutton2000policy,levine2018reinforcement}.

%We will see that action selection formulas (\ref{eq:azselection},\ref{eq:uctselection}) are closely related to local regularized policy optimization (\ref{eq:po_opt}) when the regularization terms are special instances of the Bregman divergence \citep{bregman1967relaxation}.

%\paragraph{Bregman divergence as regularizations.}
%Consider a strictly convex and differentiable convex function on the simplex $\Psi: \mathcal{S} \mapsto \mathbb{R}$. Then the associated Bregman divergence $B_\Psi : \mathcal{S}^2 \mapsto \mathbb{R}$ is defined as 
%\begin{align}
 %   B_\Psi(\mathbf{x},\mathbf{y}) = \Psi(\mathbf{x}) - \Psi(\mathbf{y}) - \nabla_y\Psi(\mathbf{y})^T(\mathbf{x}-\mathbf{y}),
%\end{align}
%where $\mathbf{x},\mathbf{y} \in \mathcal{S}$. In general, we can set $\mathcal{R}(\mathbf{y},\pi_\theta) = \Psi(\mathbf{y},\pi_\theta)$. Here, we are particularly interested in the  Bregman divergences defined by the two convex functions below \footnote{These two divergences are related to Tsallis entropy, see \citep{tsallis1988possible}}
%\begin{align}
 %   &B_0(\mathbf{x},\mathbf{y}) \eqdef \sum_i \mathbf{y}_i \log \frac{\mathbf{x}_i}{\mathbf{y}_i} = \mathbb{KL}(\mathbf{y},\mathbf{x}), \\
  %  &B_{1/2}(\mathbf{x},\mathbf{y}) \eqdef \frac{1 - \sum_i\sqrt{\mathbf{x}_i\cdot \mathbf{y}_i}}{2}.
%\end{align}



%\todoin{Yunhao: we might delay the discussion of how Qs are estimated here to the section of model-free/model-based\\ JB: Yes I think we should put it in 3.2}


%\todoin{Yunhao: do we need to discuss its connection to mirror descent? I do not think it is that necessary here as we do not use properties of mirror descent from here onwards?\\
%JB: Yes agree}


%Regularized policy optimization is similar to mirror descent in that it optimizes a linear approximation of the objective \cite{sutton2000policy} under a regularization constraint. 
% Indeed using the policy gradient theorem and noting $\mathcal{J}$ the sum of reward under policy $\pi$
% \begin{align}
%     \nabla_\theta \mathcal{J} = \mathbb{E}_x\brkt{{\mathcal{Q}_x} ^T \nabla_\theta \pi_x}
% \end{align}
% where the expectation is taken on the stationary distribution of states under policy $\pi$.  
%Indeed, in order to find a policy which maximize future reward, a large class of RL algorithm involve solving the following convex optimization problem
%\begin{align}
%\argmin_{\mathbf{y} \in \mathcal{S}}  \mathcal{Q}^T \mathbf{y} - \mathcal{R}\prth{\mathbf{y}, \pi_\theta},
%\label{eq:po_opt}
%\end{align}
%where $\mathcal{Q}$ is an estimation of the Q-values of the current policy, $\mathcal{S}$ is the $|\mathcal{A}|-$dimensional simplex and $\mathcal{R}$ a convex regularization term. 

%The intuition of the constrained optimization problem \cref{eq:po_opt} is clear - if we consider $Q^T \mathbf{y}$ as the expected gain under distribution $\mathbf{y}$, we seek a distribution $\mathbf{y}$ which maximizes the gains under some regularization constraint, for instance staying close to the prior distribution $\pi_\theta$. 

%This is exactly the motivation behind trust region policy search \citep{schulman2015trust,schulman2017proximal,abdolmaleki2018maximum,song2019v}. In these prior works, the Q-functions are estimated in a model-free manner: either via cumulative sample returns \citep{schulman2015trust,schulman2017proximal} or predicted by a critic network \citep{abdolmaleki2018maximum,song2019v}. In practice, popular choices of the regularization $\mathcal{R}$ include a KL-divergence between $\mathcal{y}$ and the prior $\pi_\theta$ to enforce the trust region \citep{schulman2015trust}; or the entropy of $\mathbf{y}$ to encourage exploration \cite{ziebart2010modeling, fox2015taming, o2016combining, haarnoja2017reinforcement}. 

==> recycle bin/old_section_3.tex <==
\section{MCTS as Policy Optimization}
\label{sec:POZero}
\todoin{Yunhao: do we want to add some motivation here? It seems to me that directly talking about $\pibar$ sounds a bit abrupt. We might want a smoother transition ici?}

\todoin{In this section we introduce $\pibar$, a quantity directly coming from policy optimization and show how $\pibar$ actually relates to the AlphaZero action selection formula. Indeed crucial to the AlphaZero algorithm is the improved policy $\pihat$ and we show that $\pibar$ we introduce below can be interpreted as a continuous relaxation of $\pihat$. }

\subsection{Notation}
Before diving in let us define some additional notations. We first define an empirical visit count $\pihat$ where an additional visit count is added to each action
\begin{align}
    \pihat(a|x) \eqdef \frac{1 + N(x,a)}{|\mathcal{A}| + \sum_{b} N(x,b)}.
    \label{eq:pihat}
\end{align}
Further, let  
\begin{align}
    \lambda \eqdef c\cdot\frac{\sqrt{\sum_b N(x,b)}}{|\mathcal{A}| + \sum_b N(x,b)}.
\end{align}
With these notations, the action selection formula (\ref{eq:azselection}) can be written as
\begin{align}
    \argmax_a Q(x,a) + \lambda \cdot \frac{\pi_\theta(a|x)}{\pihat(a|x)}.
    \label{eq:az_act_select_reformalized}
\end{align}

We also introduce vector notations to simplify the presentation. For example, we use the bold font  $\mathbf{q} \in \mathbb{R}^{|\mathcal{A}|}$ to denote the vector of search Q-function $Q(x,a)$ such that $\mathbf{q}[a] = Q(x,a)$. Similarly, when contexts are clear $\pi_\theta$ could denote either the vector $\mathbf{\pi}_\theta\in \mathbb{R}^{|\mathcal{A}|}$ or the abstract policy $\pi_\theta$. For two vector $\mathbf{u}, \mathbf{v}$ we note $\prth{\frac{\mathbf{u}}{\mathbf{v}}}[a] = \frac{\mathbf{u}[a]}{\mathbf{v}[a]}$. For convenience we sometimes remove the notation's dependency on state $x$.
We are now ready to define $\mathbf{\pibar}$ as the vector solution to the following constrained optimization problem,

\begin{align}
\pibar \eqdef \argmin_{\mathbf{y} \in \mathcal{S}}  \mathbf{q}^T \mathbf{y} - \lambda \mathbb{KL}\brkt{\pi_\theta, \mathbf{y}},
\label{eq:pibar}
\end{align}
where as in \cref{eq:po_opt}, $\mathcal{S}$ is the $|\mathcal{A}|-$dimensional simplex and $\mathbb{KL}[\cdot,\cdot]$ is the KL-divergence such that $\mathbb{KL}[\mathbf{x},\mathbf{y}] = \sum_{i} \mathbf{x}[i] \log (\mathbf{x}[i] / \mathbf{y}[i])$\todo{JB: Do we need to define the KL? Also I think I prefer just KL instead of mathbb(KL)}. See how this \cref{eq:pibar} relates to the policy optimization solution defined in \cref{eq:po_opt} where $\mathcal{Q}$ is explicitly set to the Q-values computed by the search and the KL-divergence term correspond the regularization $\mathcal{R}$. 

Note that because $\lambda$ is a decreasing function of the number of simulation gone through $x$ ebhaving as $O\prth{1/\sqrt{\sum_b N(x,b)}}$. This means that the regularization gets weaker as the number of simulation increase which makes $\pibar$ rely more and more on search Qvalues $\mathbf{q}$ and less and less on the policy prior $\pi_\theta$.

\subsection{The AlphaZero case}
The empirical visit count which is used as an improved policy by AlphaZero depends on the action selection formula which in the case of AlphaZero was handcrafted\footnote{Yet inspired by the bandit literature \cite{rosin2011multi}. } to work well on actual RL problems. 
Surprisingly we will exhibit how this $\pihat$ as defined with the AlphaZero action selection formula closely relates to $\pibar$ which was independently defined in the policy optimization literature. 
Indeed we now show how the empirical visit count $\pihat$ as defined in \cref{eq:pihat} is tracking the soft-max over search Q-values $\pibar$ defined in \cref{eq:pibar}. We first show that we can rewrite the AlphaZero action selection formula by using $\pibar$ in a way which exhibits this tracking property. 

\begin{proposition}{}
\begin{align}
\nonumber&\argmax_a \brkt{Q(x,a) + c \cdot \pi_\theta(a|x) \cdot \frac{\sqrt{\sum_b N(x,b)}}{1 + N(x,a)}} \\ 
&\quad = \argmax_a \brkt{\pi_\theta(a|x) \cdot \prth{\frac{1}{\pihat(a|x)} -  \frac{1}{\pibar(a|x)}}}
\label{eq:action_selectin_pibar}
\end{align}
\label{prop:action_selectin_pibar}
\end{proposition}

For the proof of \Cref{prop:action_selectin_pibar} see \Cref{sec:proof_action_selectin_pibar}. From this Proposition follows that the picked action $a$ is always such that $\pihat(a|x) \leq \pibar(a|x)$. This alone is enough to guarantee that $\pihat$ is tracking $\pibar$ (see \cref{sec:one_over_N_bound}). 

Not only the AlphaZero action selection formula always picks action $a$ such that $\pihat(a|x) \leq \pibar(a|x)$ but it also picks actions for which the discrepancy between $\pihat$ and $\pibar$ is the largest. Indeed we can rewrite the left term in \cref{eq:action_selectin_pibar} as $\pi_\theta \cdot \prth{\frac{1}{\pihat} -  \frac{1}{\pibar}} = \frac{\pi_\theta}{\pihat} \cdot \frac{\pibar - \pihat}{\pibar}$ where $\frac{\pibar - \pihat}{\pibar}$ is the relative difference between $\pihat$ and $\pibar$.
\todoin{comment on $\frac{\pi_\theta}{\pihat}$ term?}

The key property to prove \cref{eq:action_selectin_pibar} is the following 

\begin{align}
    \exists \alpha \forall a \quad Q(x,a) + \lambda \cdot \frac{\pi_\theta(a|x)}{\pibar(a|x)} = \alpha .
    \label{eq:relaxed_pibar}
\end{align}
This should be compared to the AlphaZero action selection formula as defined in \Cref{eq:az_act_select_reformalized}. This term comes as upper-bound on $Q$ from the bandit literature and if $Q$ is stable enough this upper-bound for a given action decreases when this action is picked. This combined with the fact that the action with the highest upperbound is always picked we can conclude that at convergence this upper-bound should be roughly constant across actions. The distribution $\pibar$ is the one for which it is exactly constant for all actions. 

The following proposition introduce an other point of view to see how $\pibar$ can be interpreted as a relaxed version of $\pihat$. 
\begin{proposition}{}
\begin{align}
\nonumber
\forall\pi\quad\mathbf{q} + \lambda \frac{\mathbf{\pi_\theta}}{\pi} = \nabla_{\pi} \prth{\mathbf{q}^T \pi - \lambda \mathbb{KL}\brkt{\mathbf{\pi_\theta}, \mathbf{\pi}}}
\end{align}
\label{prop:action_selectin_diff}
\end{proposition}

Taking $\pi = \pihat$ then the left term in Proposition~\ref{prop:action_selectin_diff} correspond to the criteria in \cref{eq:az_act_select_reformalized} that AlphaZero uses to choose actions in search. This proposition shows that the action selection formula of AlphaZero consists in picking the action in the direction which increases the most the regularized policy optimization objective for which $\pibar$ is the exact solution. 

\subsection{The UCT case}

The UCT algorithm \cite{kocsis2006bandit} is an other popular search technique with a search selection criteria based on UCB. Contrary to AlphaZero its action selection formula does not involve a prior yet we propose to include a prior and the original UCT algorithm is recovered by taking $\pi_\theta$ to be uniform. The UCT action selection formula including a prior goes as follows
\begin{align}
    \argmax_a \brkt{Q(x,a) + c \cdot \sqrt{\pi_\theta(a|x)\cdot\frac{\log\prth{\sum_b N(x,b)}}{1 + N(x,a)}}\;}.
    %\cdot \nonumber \\(c_1 + \log (\frac{\sum_b N(x,b) + c_2 + 1}{c_2}))]. 
    \label{eq:uctselection}
\end{align}

As for the AlphaZero action selection formula we can introduce $\pibar_\text{UCT}$, a soft-max over search Q-values, which is tracked by the UCT visit counts. 

\begin{align}
\pibar_\text{UCT} = \argmin_{\mathbf{y} \in \mathcal{S}}  \mathbf{q}^T \mathbf{y} - \lambda_\text{UCT} B_{1/2}\prth{\mathbf{y}, \pi_\theta},
\label{eq:pibar_uct}
\end{align}

\begin{align}
    \text{where}\quad B_{1/2}(x,y) \eqdef \frac{1 - \sum_i\sqrt{x_i\cdot y_i}}{2}
\end{align}
is a Bregman divergence associated to a Tsallis entropy\footnote{see \cref{sec:tsallis_bregman} for more detail on this} \citep{bregman1967relaxation, tsallis1988possible} and 
\begin{align}
    \lambda_\text{UCT} \eqdef c\cdot\sqrt{\frac{\log \sum_b N(x,b)}{|A| + \sum_b N(x,b)}}.
\end{align}
As for AlphaZero, $\lambda_\text{UCT}$ behaves as $O\prth{1/\sqrt{\sum_b N(x,b)}}$ therefore the regularization gets weaker as the number of simulations increases. We can also derive tracking properties between $\pibar_\text{UCT}$ and the visit count using UCT $\pihat_\text{UCT}$ as we did for AlphaZero in \cref{prop:action_selectin_pibar, prop:action_selectin_diff}.

\begin{proposition}{}
\begin{align}
\nonumber\argmax_a \brkt{Q(x,a) + c \cdot \sqrt{\pi_\theta(a|x)\cdot\frac{\log\prth{\sum_b N(x,b)}}{1 + N(x,a)}}\;} \\ 
\nonumber= \argmax_a \brkt{\sqrt{\pi_\theta(a)} \cdot \prth{\frac{1}{\sqrt{\pihat(a)}} -  \frac{1}{\sqrt{\pibar_\text{UCT}(a)}}}} 
\end{align}
\label{prob:uct_act_pi_bar}
\end{proposition}
As with \cref{prop:action_selectin_pibar} this show that the actions $a$ selected by UCT are always such that $\pihat_\text{UCT}(a|x) |le \pibar_\text{UCT}(a|x)$ which ensure a tracking property between the two. We also have a similar property as \cref{prop:action_selectin_diff}. 

\begin{proposition}{}
\begin{align}
\nonumber\forall\pi\quad\mathbf{q} + \lambda_\text{UCT} \sqrt{\frac{\mathbf{\pi_\theta}}{\mathbf{\pi}}} = \nabla_{\pi} \prth{\mathbf{q}^T \pi - \lambda_\text{UCT} \cdot B_{1/2}\brkt{\pi, \mathbf{\pi_\theta}}}
\end{align}
\label{prob:uct_act_pi_bar_diff}
\end{proposition}
which like \cref{prop:action_selectin_diff} shows that UCT selects the actions in the direction which increase the most the objective as defined in \cref{eq:pibar_uct}. 

\subsection{Experimental validation of $\pihat$ tracking $\pibar$}

To validate the practical effects of $\pihat$ tracking $\pibar$, we carry out an illustrating experiment. We simplify the general tree search into a one-step bandit case with $|\mathcal{A}|=10$ actions, with true Q-functions $Q(a)$ initialized to be uniformly randomly initialized between $[0,1]$. The prior $P(a)$ is set to be uniform and constant $c$ is set according to \citep{silver2017mastering,schrittwieser2019mastering}. To measure the tracking effect of $\pihat \approx \pibar$, we also measure the distance between $\pihat$ and the optimal distribution $\pi_G$. Note that since $\pihat$ should achieve optimality in the limit $N\rightarrow \infty$, we expect $|\pihat - \pi_G| \rightarrow 0$. To validate that the tracking of $\pihat \approx \pibar$ is non-trivial, we expect $|\pihat - \pibar|$ to converge faster to $0$. As shown in \Cref{fig:tracking}, this is indeed the case - across almost all simulation steps, $\pibar$ tracks $\pihat$ much more closely than $\pihat$ approximates $\pi_G$. See more detailed description of the experiment in the Appendix. 
\todoin{add in appendix}

==> recycle bin/old_section_3b.tex <==
% \todoin{F: do we need this remark? \\ JB: Bilal specifically told me this remark was the most important and the thing that made him understand things (including the fact that lambda actually depend on N, maybe we should note it $\lambda_N_N$?) so I vote for maintext}

% \subsection{AlphaZero as policy optimization}
% We now analyze the action selection formula of AlphaZero (\cref{eq:azselection}). Interestingly, we show that this formula, which was handcrafted\footnote{More precisely, this heuristic can be interpreted as loosely inspired by bandit literature~\citep{rosin2011multi}, but was adapted to accommodate a prior term $\pi_\theta$.} to work well on practical RL problems and completely independently of the policy optimization literature, turns out to result in a distribution $\pihat$ that closely relates to the policy optimization solution $\pibar$. \Cref{prop:action_selection_diff,eq:action_selection_pibar} allow us to formalize this result.



% \begin{proposition}{}
% For any policies $\pihat$, $\pi_\theta$ and vector $\mathbf q$,
% \begin{align}
% \mathbf{q} + \lambda_N \frac{\mathbf{\pi_\theta}}{\pihat} = \nabla_{\pihat} \prth{\mathbf{q}^T \pihat - \lambda_N \KL\brkt{\mathbf{\pi_\theta}, \pihat}} 
% \label{eq:azselect_grad}.
% \end{align}
% \label{prop:action_selection_diff}
% \end{proposition}
% % \todoin{Yunhao: do we have a rate of convergence result here? Say the convergence is faster than just using the optimal one-hot policy to approximate $\pibar$ (the question raised by David during the presentation). 
% % JB: We have 1/N in \Cref{sec:one_over_N_bound} with 1/N being the best acheiveble rate but it is for constant q (bandit case) so we didn't include in main text. You think we should? I think the argument of David does not apply here because he was confused with $\pihat \rightarrow_{N\sim\infty}\pibar$ which we don't state in the paper. \\
% % Yunhao: I see. Do we want to briefly mention the rate of convergence result here? In the conclusion 1. and 2., we state that $\pihat$ approximates $\pibar$, should we be more precise what we mean by 'approximate' (e.g. with a rate)?}

% Notice that the left-hand side of \cref{eq:azselect_grad} corresponds to the argmax argument in \cref{eq:azselection_vector}, while the right-hand side of \cref{eq:azselect_grad} is the gradient of the policy optimization objective defining  $\pibar$ (\cref{def:pibar}), evaluated at $\pihat$. Because AlphaZero's action selection formula is deterministic, it is constrained to taking actions for an integer number of times \todoin{Yunhao: 'integer num of times...' I am not sure what this sentence tries to say?}; \Cref{prop:action_selection_diff} shows that the selected action maximizes the directional derivative of the policy optimization objective. We now provide another justification that the empirical visit distribution $\pihat$ tracks the policy optimization solution $\pibar$.

% % \todoin{F: @jb can you check if the above paragraph correctly replaces this one?

% % If one could use fractional visits it is the local best update to the action visit count in order to decrease the most the policy optimization objective defined in \cref{def:pibar}. Yet a deterministic action selection formula is limited to integers visits and therefore cannot update $\pihat$ in the direction of the gradient and has to choose one single action. The \Cref{prop:action_selection_diff} shows that AlphaZero decides to pick the action with the largest derivative of the policy optimization objective.

% % We now further confirm the above intuition that the AlphaZero search procedure ensures that the empirical visit distribution $\pihat$ tracks the policy optimization solution for which $\pibar$. This result is based on the following \Cref{prop:pihat_leq_pibar}:}

% % \begin{proposition}{}
% % \begin{align}
% % \nonumber&\argmax_a \brkt{Q(x,a) + c \cdot \pi_\theta(a|x) \cdot \frac{\sqrt{\sum_b n(x,b)}}{1 + n(x,a)}} \tag{\ref{eq:azselection}} \\ 
% % = &\ \argmax_a \brkt{\pi_\theta(a|x) \cdot \prth{\frac{1}{\pihat(a|x)} -  \frac{1}{\pibar(a|x)}}}
% % \label{eq:action_selection_pibar}
% % \end{align} 
% % \label{eq:action_selection_pibar}
% % \end{proposition}

% % From which we deduce the following corollary\footnote{The proofs of \Cref{eq:action_selection_pibar} and \Cref{prop:pihat_leq_pibar} are detailed in  \Cref{sec:proof_action_selection_pibar}.}:
% % \begin{corollary}{}
% % The action $a^\ast$ realizing \cref{eq:action_selection_pibar} is such that 
% % \begin{align}
% % \pihat(a^\ast|x) \leq \pibar(a^\ast|x).
% % \end{align}
% % \label{prop:pihat_leq_pibar}\end{corollary}
% % When choosing an action $a^\ast$, $\pihat(a^\ast|x)$ increases while $\pihat$ decreases for all other actions. Therefore, if $\pibar$ is stable enough, choosing actions for which the empirical visit distribution $\pihat(a^\ast|x)$ is lower than the target distribution $\pibar(a^\ast|x)$ is a very reasonable strategy when trying to track a distribution $\pibar$. Actually, we show in \Cref{sec:one_over_N_bound} that under the constant $Q$ assumption \Cref{prop:pihat_leq_pibar} guarantees that $\pihat$ is tracking $\pibar$, with the following inequality $||\pibar - \pihat||_{\infty} \le \frac{|\mathcal{A}| + 1}{|\mathcal{A}|+N}$. 

% % Note that we can get some additional insight on AlphaZero's action selection formula by slightly rewriting the $\argmax$ argument in \cref{eq:action_selection_pibar} as \[\pi_\theta \cdot \prth{\frac{1}{\pihat} -  \frac{1}{\pibar}} = \frac{\pi_\theta}{\pihat} \cdot \frac{\pibar - \pihat}{\pibar}.\] This shows that AlphaZero not only selects action $a^\ast$ such that $\pihat(a^\ast|x) \leq \pibar(a^\ast|x)$, but it also ensures that $a^\ast$ maximizes the relative difference $\frac{\pibar - \pihat}{\pibar}$ between $\pihat$ and $\pibar$. 

% First, we have the following Proposition:
% \begin{proposition}{}
% The action $a^\ast$ realizing \cref{eq:azselection} is such that 
% \begin{align}
% \pihat(a^\ast|x) \leq \pibar(a^\ast|x).
% \end{align}
% \label{prop:pihat_leq_pibar}\end{proposition}

% To interpret \Cref{prop:pihat_leq_pibar}, remember that when sampling a new action $a^\ast$, $\pihat(a^\ast|x)$ increases (thus getting closer to $\pibar(a^\ast|x)$ for small enough increment), and $\pihat(a|x)$ decreases for all $a \neq a^\ast$. Furthermore, the step size by which $\pihat$ changes when a new action is taken decreases as $\frac{1}{N}$. If $\pibar$ remains stable enough, this dynamics eventually leads results in $\pihat$ tracking $\pibar$; in \Cref{sec:one_over_N_bound}, we establish an even stronger tracking result, namely that under a constant $Q$ assumption\footnote{This result assumes that the value of $Q(x, a)$ does not change over time, which is not the case in MCTS; we leave the extension of this theoretical result to MCTS-like settings to future work.}, \Cref{prop:pihat_leq_pibar} guarantees that $||\pibar - \pihat||_{\infty} \le \frac{|\mathcal{A}| + 1}{|\mathcal{A}|+ \mathcal N}$.

% To obtain the inequality of \Cref{prop:pihat_leq_pibar}, we prove in \Cref{sec:proof_action_selection_pibar} that
% \begin{align}
% \nonumber&\argmax_a \brkt{Q(x,a) + c \cdot \pi_\theta(a|x) \cdot \frac{\sqrt{\sum_b n(x,b)}}{1 + n(x,a)}} \tag{\ref{eq:azselection}} \\ 
% = &\ \argmax_a \brkt{\pi_\theta(a|x) \cdot \prth{\frac{1}{\pihat(a|x)} -  \frac{1}{\pibar(a|x)}}}. 
% \label{eq:action_selection_pibar}
% \end{align}
% Then, because $\sum_a \pihat(a|x) = \sum_a \pibar(a|x)$ and $\pihat >0$ and $\pibar >0$, there exists at least one action for which $0 < \pihat(a|x) \leq \pibar(a|x)$, \emph{i.e.} $\frac{1}{\pihat(a|x)} - \frac{1}{\pibar(a|x)} \geq 0$. 

% % \Cref{eq:action_selection_pibar} shows that AlphaZero selects the action $a^\ast$ in order to maximize the relative difference $\frac{\pibar - \pihat}{\pibar}$ between $\pihat$ and $\pibar$. For this reason, we say that \emph{$\pihat$ is tracking $\pibar$}; in \Cref{sec:one_over_N_bound}, we establish an even stronger tracking result, namely that under a constant $Q$ assumption\footnote{This result assumes that the value of $Q(x, a)$ does not change over time, which is not the case in MCTS; we leave the extension of this theoretical result to MCTS-like settings to future work.}, \Cref{prop:pihat_leq_pibar} guarantees that $||\pibar - \pihat||_{\infty} \le \frac{|\mathcal{A}| + 1}{|\mathcal{A}|+N}$.

% % \todoin{F: do we want to keep this? If so, we probably need a plot or something..

% % When choosing an action $a^\ast$, $\pihat(a^\ast|x)$ increases while $\pihat$ decreases for all other actions. Therefore, if $\pibar$ is stable enough, choosing actions for which the empirical visit distribution $\pihat(a^\ast|x)$ is lower than the target distribution $\pibar(a^\ast|x)$ is a very reasonable strategy when trying to track a distribution $\pibar$. Actually, we show in \Cref{sec:one_over_N_bound} that under the constant $Q$ assumption \Cref{prop:pihat_leq_pibar} guarantees that $\pihat$ is tracking $\pibar$, with the following inequality $||\pibar - \pihat||_{\infty} \le \frac{|\mathcal{A}| + 1}{|\mathcal{A}|+N}$. 

% % Note that we can get some additional insight on AlphaZero's action selection formula by slightly rewriting the $\argmax$ argument in \cref{eq:action_selection_pibar} as \[\pi_\theta \cdot \prth{\frac{1}{\pihat} -  \frac{1}{\pibar}} = \frac{\pi_\theta}{\pihat} \cdot \frac{\pibar - \pihat}{\pibar}.\] This shows that AlphaZero not only selects action $a^\ast$ such that $\pihat(a^\ast|x) \leq \pibar(a^\ast|x)$, but it also ensures that $a^\ast$ maximizes the relative difference $\frac{\pibar - \pihat}{\pibar}$ between $\pihat$ and $\pibar$. }

% From both \Cref{prop:action_selection_diff,prop:pihat_leq_pibar} we deduce:

% \begin{conclusion}{}
% AlphaZero's search policy $\pihat$ approximates the exact solution $\pibar$ of the regularized policy optimization problem of \cref{def:pibar}.\label{thm:az_is_approximate_po}
% \end{conclusion}

==> recycle bin/old_section_4.tex <==
\section{Algorithms}
\label{sec:algo}

\todoin{Make notations clearer re "MCTS"}

In this section we propose algorithmic improvements based on insights of the previous section. In particular, recall that we have defined $\pibar$, a soft-max distribution over search Q-values. Further, we have showed how the empirical visit distribution $\pihat$ tracks $\pibar$ as much as possible. Below, we will first argue why using $\pibar$ in place of $\pihat$ is in general preferable and then we will see how to actually apply $\pibar$ as a better alternative to $\pihat$. 

\subsection{Advantages of using $\pibar$ over $\pihat$}
\label{sec:mcts_as_po-motivation}
When simulation budgets are low (i.e. small $n_{\text{sim}}$), AlphaZero could misbehave. Indeed because the visit count is discrete and the action selection deterministic, the visit count fails to properly account for the information contained in the Q-function estimate. In the extreme case of one simulation the selected action is just the one with the largest prior completely ignoring the Q-function estimate. In general in the first few simulations during initial simulations of the search, the visit count at the root $N(x_0, a)$ concentrates around the mode of the prior and does not absorb much information from the Q-function $Q(x,a)$. As a result, the learning  target $\pihat_{\text{mcts}}(a|x)$ does not generate an optimized local policy and hardly improves the parametric policy $\pi_\theta(a|x)$. 

Also note that when the Q-function estimates are updated, $\pibar$ immediately adjust accordingly contrary to the visit count $\pihat$ that has to rely on future simulation to get updated.  

Another advantage of using $\pibar$ in place of $\pihat$ is to decouple the search strategy at the root from the learning target. In AlphaZero any change on the action selection formula can heavily affect $\pihat$ which is used both as a policy and as training target. Instead $\pibar$ only depends on the $Q$-values estimated by search. Therefore using $\pibar$ allows to use quite different action selection strategy at the root, even very exploratory ones without affecting the training targets and the policy.  

\todoin{Yunhao: wdyt put the sim - performance plot on ms acpman (run by Thomas) here? This helps illustrate the idea that $\pihat$ misbehaves with small num sims? Also, we have quite many words across these several pages, having some plots here might refresh the reviewers a bit as well?}

% \todoin{some simple mdp/bandit example here and plots. JB: What do you have in mind more specifically?}

% % How do we extend AlphaZero such that the algorithm performs reliably even under small simulation budgets? Instead of making ad-hoc changes, below we start by analyzing how AlphaZero selects actions during search. We will see that under the seemingly arbitrary design choices of AlphaZero, in particular the action selection formula \cref{eq:azselection}, there already exists a principled way to improve the algorithm.

% \todoin{small experiments that show pi bar works with small simulation budgest. JB: Don't you think our experiments on muZero atari/control are enought, what do you have in mind? Like a tabular random mdp? Yunhao: I tried some small mdps and it does not seem to work that well (maybe bugs), but yeah I think the current experiments should suffice.}

%\subsection{Connections between AlphaZero and model-free policy optimization. }

\subsection{Proposed AlphaZero modifications}
In AlphaZero $\pihat$ is used in three different places: learning, search and acting. We propose to replace $\pihat$ by $\pibar$ in these three places and we refer to \algoall{} for AlphaZero with the three following modifications. 
\paragraph{\algoact{}: acting with $\pibar$.}
AlphaZero selects the action to execute in the real world by sampling proportionally to the visit count $a\sim\pihat(\cdot|x_\text{root})$. Instead, we propose to select the action by sampling according to $\pibar(\cdot|x_\text{root})$ and name this modification \algoact{} in the following of the paper. 
\paragraph{\algolearn{}: learning with $\pibar$.} [hi florent, je te vois]
Since the search is meant to generate an optimized local policy, ideally we should expect the empirical visit count to improve upon e.g. the prior $\pi_\theta(a|x)$. However, this local policy is represented in a tabular way and does not allow for generalization to other unseen states. To distill the knowledge of the local policy into the parametric policy, AlphaZero reduces the expected KL-divergence by gradient between the prior distribution and the visit count descent on the network parameters $\theta$. We instead we propose to distill $\pibar$ into the prior network and name this modification \algolearn{} in the following. 
\begin{align}
    \mathbb{E}_{x_\text{root}}\Big[\mathbb{KL}\brkt{\pibar(\cdot|x), \pi_\theta(\cdot|x_\text{root})}\Big],
    \label{eq:azlearning}
\end{align}
where $x_\text{root}$ is sampled from a distribution over states\footnote{e.g., from a prioritized replay buffer like in MuZero \citep{schrittwieser2019mastering}.}. 
\paragraph{\algosearch{}: searching with $\pibar$.}
During the search, instead of selecting actions according to \cref{eq:azselection}, we propose to  instead sample actions according to $\pibar$. Instead of using a UCB like algorithm to recursively decide a path in a tree this  modification is similar to using a mirror descent type of bandit algorithm. In this modification each node store its own Q-function estimate $Q$ and visit count $N$ like in AlphaZero but additionally compute its own $\pibar$ and update it during the MCTS back-propagation phase. We name this modification \algosearch{} in the following.

See \Cref{fig:pz_ablation} for an ablation study.

\begin{figure}[h]
\begin{subfigure}{0.95\columnwidth}
\includegraphics[width=\linewidth]{plots/ablation/ablation_5_sims_per_seed.pdf}\caption{\label{fig:pz_ablation_5_sims}5 simulations}
\end{subfigure}

\begin{subfigure}{0.95\columnwidth}
\includegraphics[width=\linewidth]{plots/ablation/ablation_50_sims_per_seed.pdf} \caption{\label{fig:pz_ablation_50_sims} 50 simulations}
\end{subfigure}
\caption{\label{fig:pz_ablation}Ablation study from \algoall{} at 5 and 50 simulations per step.}
\end{figure}

%\subsection{Bridging AlphaZero and model-free policy optimization. (Connections between AlphaZero and model-free policy optimization.)}

\subsection{Interpreting AlphaZero as Policy Optimization}

%By construction, AlphaZero and model-free policy optimization algorithms take very distinct formulations. Indeed, at the first glance, AlphaZero relies on model-based planning while model-free policy optimization relies on local model-free policy improvement. We will see below that by extending AlphaZero to \algoall{} (\algoact{} + \algolearn{} + \algosearch{}), we bridge the conceptual gap between these two paradigms.

We will see below that when extending AlphaZero to \algoall{}, we could provide an interpretation of the new algorithm as policy optimization. This interpretation allows us to make connections to prior works and opens door to new algorithmic variants.

Recall that \algoall{} contains three main parts: \algoact{}, \algolearn{} and \algosearch{}. The exact interpretation depends on how we abstract the algorithm, i.e. whether we treat an algorithmic component as blackbox. We provide two consistent interpretations below.

\paragraph{\algolearn{} as Policy Optimization.} For this interpretation, we treat \algosearch{} as a blackbox, i.e. as a subroutine that takes a root node $x$ and returns statistics such as search Q-values $Q(x,a)$.

Recall that model-free policy optimization (eq. (\ref{eq:po_opt})) roughly consists in optimizing the objective $\mathcal{Q}_{\pi_\theta}^T \mathbf{y}$ with local policy $\mathbf{y}$. There is a spectrum of model-free approaches to estimating $\mathcal{Q}_{\pi_\theta}$: at one end of the spectrum, the estimate builds on Monte-Carlo samples of cumulative returns $\mathcal{Q}^{\pi_\theta}\approx \sum_{t\geq 0} r_t\gamma^t$ \citep{schulman2015trust,schulman2017proximal}\footnote{More accurately, we note that \citet{schulman2015trust,schulman2017proximal} also blends the estimates with value function critic $v_\theta$ for bias-variance trade-off.}; at another end, the estimate is predicted from a Q-value critic $\mathcal{Q}_{\pi_\theta} \approx \mathbf{q}_\theta$, trained on off-policy samples \citep{abdolmaleki2018maximum,song2019v}. 

As a result, we can interpret \algolearn{} as policy optimization based on eq. (\ref{eq:po_opt}), with $\mathcal{Q}_{\pi_\theta}$ estimated via tree search. Indeed, \algolearn{} $+$ \algoact{} could be interpreted as building Q-function\footnote{During search, because child nodes have fewer simulations than the root, the Q-function estimate at the root slightly under-estimates the acting policy Q-function.} critics $\mathbf{q}_\theta$ with a tree-structured inductive bias. However, this inductive bias is not an architectural built-in \citep{silver2017predictron,farquhar2017treeqn,oh2017value}, but constructed online by an algorithm, i.e. MCTS. 

The idea of model-based estimations for model-free RL is not new, prior works \citep{feinberg2018model,buckman2018sample,hamrick2019combining} have applied similar ideas to Q-learning. However, here within the framework of policy optimization, the transition between model-free and model-based RL becomes more smooth and clear.

\paragraph{\algosearch{} as Policy Optimization.} For this interpretation, we unpack the tree search blackbox and interpret it as policy optimization. 

Specifically, during forward simulations, at each child node $x$, the action is selected from $a \sim \pibar (\cdot|x)$. As a result, the full imaginary trajectory is generated consistently according to policy $\pibar$. Then during backward updates, each encountered node $x$ receives a backup value from its child node, which is an exact estimate of $Q^{\pibar}(x,a)$. Finally, the local policy $\pibar(a|x)$ is updated via the constrained optimization (eq. (\ref{eq:pibar})). Overall, the \algosearch{} optimizes the policy (and Q-function) at the root node, by solving a sequence of local policy optimization problems across the entire search tree\footnote{Note that there are several differences from typical model-free implementations of policy optimization: for example, unlike a fully-parameterized policy, the tree search policy is tabular at each node.}

From this perspective, the \algosearch{} is a blackbox subroutine that distills the improved policy $\pibar$ into $\pi_\theta$. While \algosearch{} obtains such improved policy $\pibar$ via a sequence of regularized policy optimization, other alternatives exist. For example, since $\pihat$ approximates $\pibar$, AlphaZero obtains the approximate improved policy $\pihat$ via MCTS (eq. (\ref{eq:azselection})). Alternatively, the tree search could be replaced by policy gradients \citep{anthony2019policy} or evolutionary strategies \citep{chua2018deep}.
